Understanding the Motivations, Challenges and Needs of Blockchain Software Developers: A Survey

The blockchain technology has potential applications in various areas such as smart-contracts, Internet of Things (IoT), land registry, supply chain management, storing medical data, and identity management. Although the Github currently hosts more than six thousand active Blockchain software (BCS) projects, few software engineering research has investigated these projects and its' contributors. Although the number of BCS projects is growing rapidly, the motivations, challenges, and needs of BCS developers remain a puzzle. Therefore, the primary objective of this study is to understand the motivations, challenges, and needs of BCS developers and analyze the differences between BCS and non-BCS development. On this goal, we sent an online survey to 1,604 active BCS developers identified via mining the Github repositories of 145 popular BCS projects. The survey received 156 responses that met our criteria for analysis. The results suggest that the majority of the BCS developers are experienced in non-BCS development and are primarily motivated by the ideology of creating a decentralized financial system. Although most of the BCS projects are Open Source Software (OSS) projects by nature, more than 93% of our respondents found BCS development somewhat different from a non-BCS development as BCS projects have higher emphasis on security and reliability than most of the non-BCS projects. Other differences include: higher costs of defects, decentralized and hostile environment, technological complexity, and difficulty in upgrading the software after release. Software development tools that are tuned for non-BCS development are inadequate for BCS and the ecosystem needs an array of new or improved tools, such as: customized IDE for BCS development tasks, debuggers for smart-contracts, testing support, easily deployable simulators, and BCS domain specific design notations.

==> Sections/industry-comparison.tex <==
%\resizebox{0.95\linewidth}{!} {
\resizebox{\linewidth}{!} {
\begin{tabular}{|l|p{7.5cm}|p{1.7cm}|r|r|r|r|r|r|}
\hhline{---------}
&\multirow{2}{*}{\textbf{Statement}}  &  \multirow{2}{1.7cm}{\textbf{Rating\newline distribution}} & \multicolumn{2}{c}{\textbf{BCS Vs. Games}} & \multicolumn{2}{|c}{\textbf{BCS Vs. Office}} & \multicolumn{2}{|c|}{\textbf{BCS Vs. Other}} \\ \hhline{~~~------}
& & & $p$  & $r$ & $p$ & $r$  &$p$ & $r$ 
\\ \hhline{-|-|-|-|-|-|-|-|-|}

\multicolumn{9}{l}{ \hspace*{1cm}\textbf{ A. Quality assurance}}\\ \hline


 


QA1.& My software is well tested manually (e.g., paid testers thoroughly use the software).&  \ticker{.9}{11}{30.3}{41.3}{16.5}
 & 0.82 &\moren{ 0.06} &  \significant{ 0.02} & \less{ 0.14} &  \significant{ 0.04} &  \more{0.12} \\ \hhline{-|-|-|-|-|-|-|-|-|}


QA2.& My software is well tested by automated testing (e.g., scripts that thoroughly use the software).&  \ticker{2.8}{8.3}{19.3}{45.9}{23.9}
 &  \significant{ $<0.01$ }& \more{ 0.32} & \significant{0.04} & \more{ 0.12} &  \significant{ $<0.01$} &\more{ 0.18} 
 \\ \hhline{-|-|-|-|-|-|-|-|-|}
 
 
QA3.& My software is well tested by unit tests.&  \ticker{2.8}{11.0}{18.3}{47.7}{20.2}
 &  \significant{ $<0.01$} &\more{ 0.34} & \significant{ $<0.01$} & \more{0.31} & 0.45 &\moren{ 0.01} \\ \hhline{-|-|-|-|-|-|-|-|-|}

QA4.& Bugs in my software are hard to diagnose. &  \ticker{4.6}{26.6}{33.0}{32.1}{3.7}
&  \significant{ $<0.01$} & \more{ 0.23} & 0.12 & \moren{ 0.08} & 0.2 & \moren{ 0.06} \\ \hhline{-|-|-|-|-|-|-|-|-|}

QA5.& It's difficult to write thorough automated tests for my software because it's so complex.&   \ticker{8.3}{34.3}{27.8}{25}{4.6}
 &  \significant{ 0.01} & \less{ 0.15} & 0.08 &\lessn{ 0.1} & 0.93 & \lessn{0.1} \\ \hhline{-|-|-|-|-|-|-|-|-|}
 
 
%S1.& Most of the code I write is reviewed by other people. &  \ticker{7.3}{6.4}{10.9}{29.1}{54.6}
% &  \significant{ 0.02} & \less{ 0.13} &  \significant{ $<0.01$} &\less{ 0.33} & \significant{ $<0.01$} & \less{ 0.25} \\ \hhline{-|-|-|-|-|-|-|-|-|}


\multicolumn{9}{l}{\hspace*{1cm}\textbf{B. Development process}}\\ \hline

DP1.& My team has flexible release deadlines.&  \ticker{3.7}{8.3}{17.4}{45.9}{24.8}
 &  \significant{ $<0.01$} & \more{ 0.46} &  \significant{ $<0.01$} &\more{ 0.53} &   \significant{ $<0.01$} &\more{ 0.44}

\\ \hhline{-|-|-|-|-|-|-|-|-|}

DP2.& My software has clear functional requirements.&  \ticker{1.8}{7.3}{21.8}{49.1}{20}
 & \significant{ 0.01} & \more{ 0.14} & 0.62 &\lessn{ 0.02} & 0.91 &\moren{ 0.09} \\ \hhline{-|-|-|-|-|-|-|-|-|}
 
 DP3. &My team uses a waterfall process, rather than an agile process.&  \ticker{30}{32.7}{30}{7.3}{0}
 &   \significant{ 0.03} & \more{ 0.12} & 0.65 &\lessn{ 0.03} &  0.07 & \lessn{ 0.08} \\ \hhline{---------}
DP4.& My team adheres strictly to a process (for example, scrum or waterfall).&  \ticker{19.3}{33.9}{26.6}{15.6}{4.6}
 &  \significant{ $<0.01$} & \less{ 0.2} &  \significant{ $<0.01$} & \less{ 0.37} & \significant{ $<0.01$} & \less{ 0.29} \\ \hhline{---------}
 
 
%S4.& Most of the feature code I write will probably be included in the shipped software.&  \ticker{.9}{4.6}{13.8}{51.4}{29.4}  & 0.44 & \moren{ 0.01} & 0.26 & \moren{ 0.05} &  0.12 & \lessn{0.08} \\ \hhline{-|-|-|-|-|-|-|-|-|}
 
 \multicolumn{9}{l}{\hspace*{1cm}\textbf{C. Software maintenance}}\\ \hline
 
 SM1.& My software has high technical debt (for example, a lot of hacks). &  \ticker{19.1}{40}{26.4}{10.9}{3.6} 
 & 0.27 &\lessn{ 0.04} & 0.08 &\lessn{ 0.1} & 0.39 &\lessn{ 0.02} \\ \hhline{-|-|-|-|-|-|-|-|-|}

SM2.& The technical debt is likely to be paid down in the future (for example, through refactoring).&  \ticker{1.8}{13.6}{29.1}{41.8}{13.6}
 &  \significant{ $<0.01$} &\more{ 0.18} & \significant{ $<0.01$} & \more{ 0.23} &  \significant{ 0.01} & \more{ 0.17} \\ \hhline{-|-|-|-|-|-|-|-|-|}
 
 SM3.& My software's architecture evolves significantly as the software gets more mature.&  \ticker{.9}{9.1}{15.5}{55.5}{19.1}
 & 0.23 & \moren{ 0.05} &   0.06 & \moren{ 0.09} & 0.32 & \moren{ 0.03} \\ \hhline{-|-|-|-|-|-|-|-|-|}

 


 \multicolumn{9}{l}{\hspace*{1cm}\textbf{D. Ideology / morale} }\\ \hline


 DM1.& My software creates value for society.&  \ticker{0}{0}{15.7}{40.7}{43.5}
 &  \significant{ $<0.01$} &\more{ 0.26} & 0.15 &\moren{ 0.07} &  \significant{ 0.01} &\more{ 0.17} \\ \hhline{-|-|-|-|-|-|-|-|-|}

DM2.& Creativity is highly valued on my team.&  \ticker{.9}{3.7}{25.7}{43.1}{26.6}
 &  \significant{ 0.02} & \less{ 0.14} & 0.4 & \moren{0.02} & 0.36 &\moren{ 0.02} \\ \hhline{-|-|-|-|-|-|-|-|-|}
%S10.& Creating my software requires a team of people, each with different skills.&  \ticker{4.6}{10.1}{15.6}{36.7}{33}
% &  \significant{ $<0.01$} & \less{ 0.2} & 0.36 &\lessn{ 0.03} & 0.55 &\lessn{ 0.01} 
 
%  \\ \hhline{-|-|-|-|-|-|-|-|-|}


DM3.& Creating my software is challenging.&  \ticker{.9}{8.3}{13.9}{54.6}{22.2}
 & 0.19 & \lessn{ 0.06} & 0.5 &\lessn{ 0} & 0.66 & \lessn{0.03} \\ \hhline{-|-|-|-|-|-|-|-|-|}
DM4.& When I tell people outside of my company about the software I work on, they are impressed.&  \ticker{.9}{1.9}{24.1}{50.9}{22.2}
 & \significant{ 0.03} &\less{ 0.13} & 0.07 & \moren{0.1} &  \significant{ 0.05} &\more{ 0.11} \\ \hhline{-|-|-|-|-|-|-|-|-|}


\end{tabular} 
}

==> Sections/project-list.tex <==
\resizebox{\linewidth}{!} {
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline 
\multicolumn{3}{|c|} { \graycell{Multiple occurences}} & \multicolumn{4}{c|}  { \graycell{ Single occurences}} \\ 
\hline 
Ethereum (22) & Bitcoin (9)  & Bitshares (7) & Ambisafe & Basic Identity Token & Bytom & Cpuminer
\\ \hline
Monero (6) & Sia (6) & Waves (5) & Dash & Distense &  DNSChain & Ebets 
\\ \hline
Solidity (5) & Lbry (4) & Ripple (4) & ESKU & Etherbet &Etherplay & Fabric Labs
\\ \hline
Nem (3) & Cardano (3) & Decred (3) & Golem & Haskoin & ZeroLink & Icofunding
\\ \hline
EOS (3) & Hyperledger (3) & IOTA (3) &Ind & Iroha & JS Miner & Keyrun 
\\ \hline
Factom (2) & Feather coin (2) & Lisk (2)   & Libsnark & LiteCoin & Payroll System & PHP-Mpos   
\\ \hline
Metamask (2) & Namecoin (2) & Neo (2) & Populus & Progmathon & Pycoin & Shapeshift 
\\ \hline
Remix IDE (2) & Stratis (2) & Trezor (2) & Snapcoin & Status & Steller & Storj 
\\ \hline
 Zcash (2) & \multicolumn{2}{l|}{ Undisclosed /Private (14)} & Swifty & Vandal & Vcash & Viper
\\ \hline

\end{tabular} 
}

==> Sections/survey-questions.tex <==
%\resizebox{0.9\textwidth}{!} {
\resizebox{\linewidth}{!} {
\begin{tabular}{p{.02\textwidth}p{.02\textwidth}p{.55\textwidth}p{.35\textwidth}}
\hline
\textbf{\#} & \textbf{RQ*} & \textbf{Question Text} & \textbf{Answer Choices} \\
\hline
Q1 & RQ1 & How old are you? & [\#]  \\
Q2 & RQ1 & Which gender do you identify yourself with? & [Male, Female, Prefer not to disclose] \\ 
Q3 & RQ1 & What is your highest level of education? & [High school, Bachelors, Masters, Ph.D.] \\
Q4 & RQ1 & How many years of software development experiences do you have? & [Less than a year, between one to five years, between six to ten years, more than ten years] \\
Q5 & RQ1 & How many years have you been developing blockchain software?& [Less than a year, between one to two years, between three to five years, more than five years] \\
Q6 & RQ1 & What is your primary Blockchain software project (i.e. the project that you have spent most of your time) & [\#]  \\
&\\
Q7 & RQ1 & Do you receive any direct compensation (i.e, salary or cryptocurrency) from your primary project? & [I get directly paid with a FIAT currency, I get compensated with shares, tokens, or cryptocurrency, I receive both FIAT salary and tokens/shares, No, I do not receive any direct compensation] \\
%Q8 & D & Approximately how many developers regularly contribute to your primary project? & [less than 10, between 10 to 30, between 30 to 50, more than 50] \\
%Q9 & D & What are your roles in your primary project (please check all appropriate roles)? & [Developer, Maintainer, requirement analysis, Testing, User support, Documentation, Social marketing] \\
%&\\Q10 & D & How many other blockchain software projects have you contributed? & [\#] \\
Q8 & RQ1 & Approximately, how many pull requests have you submitted to your primary project? & [Less than 10,  Between 11 to 30, More than 30] \\
Q9 & RQ1 & Approximately, how many hours on average do you spend per week on your primary project? & [Less than 5, between 6 to 10, Between 11 to 20, Between 21 to 35, I work full time] \\
Q10 & RQ2 & What are your motivations to contribute to your primary project?  &\\
Q11 & RQ3 &  Based on your experiences, what are the primary differences between blockchain and non-blockchain software development ? & [\#]  \\
Q12 & RQ3 & \textit{ The following statements aim to compare blockchain and non-blockchain software development. For each of the following items please rate how you agree or disagree with
that statement}.& [Strongly disagree, Disagree, Neutral, Agree, Strongly Agree]  \\
&  &Total 16 statements ( shown in Table~\ref{table:comparison}) &  \\
Q13 & RQ4 & What are the most challenging aspects of blockchain software development? &\\
%Q15 & RQ3 & Which of the following channels do you use to communicate with the peers from your
%primary project? Please check all that apply. & [email, Slack, Discord, Github, instant messenger, Skype, mailing list, Reddit, Medium, others (please specify)] \\
%Q16 & RQ4 & Which of the following software development practices do you follow (Please check all that apply)? & [peer code review, automated build( aka one-click build using ANT, Maven, Gradle, CMake), continuous integration (e.g., Travis, Jenkins, Teamcity, Bamboo, Buildbot, or Cruisecontrol), pair programming, unit testing, automated testing, test driven development (aka test first development), performance testing, formal verification, others (please specify)] \\
%Q17 & RQ5 & Please rank the following software development practices based on their
%effectiveness to improve the quality of your project (you can drag and drop to reorder the
%following list): & [formal verification, automated testing, pair programming, performance testing, test driven development (aka test first development), unit testing, continuous integration (e.g., Travis, Jenkins, Teamcity, Bamboo, Buildbot, or Cruisecontrol), peer code review, automated build( aka one-click build using ANT, Maven, Gradle, CMake)] \\
%Q18 & RQ6 &  How the requirements of your projects are identified and selected? & [\#]  \\
%Q19 & RQ7 &  How development tasks are assigned among the project members? & [\#]  \\
%Q20 & RQ8 &  How do you verify the correctness of your code? & [\#]  \\
%Q21 & RQ9 &  How do you test your software for security and scalability? & [\#]  \\
%& &\textit{Comparison between blockchain and non-blockchain software development.} \\
Q14 & RQ5 &  Please describe the type of tools that you currently do not have, but if implemented, can greatly help your blockchain software development activities. & [\#]  \\
\hline
\multicolumn{4}{l}{\small{\textit{*numbers refer to the research question that motivated the inclusion of the survey question}}}
\end{tabular}
}
